Bending the Automation Bias Curve: A Study of Human and AI-based Decision Making in National Security Contexts

Uses of artificial intelligence (AI), especially those powered by machine learning approaches, are growing in sectors and societies around the world. How will AI adoption proceed, especially in the international security realm? Research on automation bias suggests that humans can often be overconfident in AI, whereas research on algorithm aversion shows that, as the stakes of a decision rise, humans become more cautious about trusting algorithms. We theorize about the relationship between background knowledge about AI, trust in AI, and how these interact with other factors to influence the probability of automation bias in the international security context. We test these in a preregistered task identification experiment across a representative sample of 9000 adults in 9 countries with varying levels of AI industries. The results strongly support the theory, especially concerning AI background knowledge. A version of the Dunning Kruger effect appears to be at play, whereby those with the lowest level of experience with AI are slightly more likely to be algorithm-averse, then automation bias occurs at lower levels of knowledge before leveling off as a respondent's AI background reaches the highest levels. Additional results show effects from the task's difficulty, overall AI trust, and whether a human or AI decision aid is described as highly competent or less competent.

==> Tables/Table3.tex <==
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                    &\multicolumn{1}{c}{\shortstack{Overall\\Binary\\b/SE}}&\multicolumn{1}{c}{\shortstack{AI Condition\\Binary\\b/SE}}&\multicolumn{1}{c}{\shortstack{Human Condition\\Binary\\b/SE}}&\multicolumn{1}{c}{\shortstack{Switching in AI Condition\\AI Familiarity Model\\b/SE}}&\multicolumn{1}{c}{\shortstack{Switching in AI Condition\\AI Background Model\\b/SE}}\\
\hline
QPolitical          &                     &                     &                     &       0.032\sym{***}&       0.034\sym{***}\\
                    &                     &                     &                     &     (0.010)         &     (0.010)         \\
Level of Difficulty &       0.034\sym{***}&       0.035\sym{***}&       0.041\sym{***}&       0.200\sym{***}&       0.200\sym{***}\\
                    &     (0.003)         &     (0.004)         &     (0.004)         &     (0.034)         &     (0.034)         \\
Practice Round Accuracy&      -0.008\sym{***}&      -0.011\sym{***}&      -0.008\sym{***}&      -0.042\sym{**} &      -0.044\sym{**} \\
                    &     (0.002)         &     (0.002)         &     (0.002)         &     (0.019)         &     (0.019)         \\
Age                 &      -0.000\sym{*}  &      -0.000\sym{**} &      -0.000         &      -0.000         &      -0.000         \\
                    &     (0.000)         &     (0.000)         &     (0.000)         &     (0.002)         &     (0.002)         \\
Gender              &       0.030\sym{***}&       0.035\sym{***}&       0.034\sym{***}&       0.225\sym{***}&       0.218\sym{***}\\
                    &     (0.004)         &     (0.006)         &     (0.005)         &     (0.049)         &     (0.050)         \\
Level of Education  &       0.005\sym{***}&       0.007\sym{***}&       0.005\sym{**} &       0.025\sym{*}  &       0.036\sym{**} \\
                    &     (0.001)         &     (0.002)         &     (0.002)         &     (0.015)         &     (0.015)         \\
Treatment Condition: AI&       0.045\sym{***}&                     &                     &                     &                     \\
                    &     (0.003)         &                     &                     &                     &                     \\
Treatment Condition: High Confidence&       0.056\sym{***}&       0.017\sym{***}&       0.016\sym{***}&       0.093\sym{***}&       0.092\sym{***}\\
                    &     (0.003)         &     (0.004)         &     (0.004)         &     (0.034)         &     (0.034)         \\
Overall AI Familiarity&                     &                     &                     &       1.928\sym{***}&                     \\
                    &                     &                     &                     &     (0.388)         &                     \\
AI Familiarity Squared&                     &                     &                     &      -1.788\sym{***}&                     \\
                    &                     &                     &                     &     (0.463)         &                     \\
AI Background Index &                     &                     &                     &                     &       1.289\sym{***}\\
                    &                     &                     &                     &                     &     (0.483)         \\
AI Background Index Squared&                     &                     &                     &                     &      -1.547\sym{**} \\
                    &                     &                     &                     &                     &     (0.653)         \\
Normalized AI Sentiment&                     &                     &                     &      -0.349\sym{**} &      -0.274\sym{*}  \\
                    &                     &                     &                     &     (0.158)         &     (0.161)         \\
Russia              &      -0.038\sym{***}&      -0.052\sym{***}&      -0.035\sym{***}&                     &                     \\
                    &     (0.008)         &     (0.011)         &     (0.011)         &                     &                     \\
China               &       0.070\sym{***}&       0.081\sym{***}&       0.077\sym{***}&                     &                     \\
                    &     (0.010)         &     (0.013)         &     (0.013)         &                     &                     \\
United Kingdom      &       0.024\sym{***}&       0.024\sym{**} &       0.028\sym{**} &                     &                     \\
                    &     (0.009)         &     (0.012)         &     (0.012)         &                     &                     \\
Australia           &       0.018\sym{**} &       0.017         &       0.025\sym{**} &                     &                     \\
                    &     (0.009)         &     (0.012)         &     (0.012)         &                     &                     \\
Japan               &      -0.032\sym{***}&      -0.032\sym{***}&      -0.040\sym{***}&                     &                     \\
                    &     (0.009)         &     (0.012)         &     (0.011)         &                     &                     \\
South Korea         &      -0.040\sym{***}&      -0.046\sym{***}&      -0.045\sym{***}&                     &                     \\
                    &     (0.009)         &     (0.012)         &     (0.011)         &                     &                     \\
France              &      -0.011         &      -0.016         &      -0.010         &                     &                     \\
                    &     (0.009)         &     (0.012)         &     (0.012)         &                     &                     \\
Sweden              &      -0.005         &      -0.007         &      -0.006         &                     &                     \\
                    &     (0.009)         &     (0.012)         &     (0.011)         &                     &                     \\
Constant            &       0.147\sym{***}&       0.219\sym{***}&       0.196\sym{***}&      -1.588\sym{***}&      -1.615\sym{***}\\
                    &     (0.011)         &     (0.015)         &     (0.015)         &     (0.167)         &     (0.180)         \\
\hline
Observations        &       90160         &       39903         &       40255         &       26214         &       26214         \\
\(R^{2}\)           &       0.020         &       0.015         &       0.014         &                     &                     \\
Pseudo \(R^{2}\)    &                     &                     &                     &       0.010         &       0.007         \\
Log Likelihood      &  -44495.143         &  -21683.412         &  -21555.620         &  -14202.630         &  -14236.006         \\
F                   &      88.738         &      26.239         &      27.421         &                     &                     \\

